Approximate Agreement under Mobile Byzantine Faults

In this paper we address Approximate Agreement problem in the Mobile Byzantine faults model. Our contribution is threefold. First, we propose the the first mapping from the existing variants of Mobile Byzantine models to the Mixed-Mode faults model.This mapping further help us to prove the correctness of class MSR (Mean-Subsequence-Reduce) Approximate Agreement algorithms in the Mobile Byzantine fault model, and is of independent interest. Secondly, we prove lower bounds for solving Approximate Agreement under all existing Mobile Byzantine faults models. Interestingly, these lower bounds are different from the static bounds. Finally, we propose matching upper bounds. Our paper is the first to link the Mobile Byzantine Faults models and the Mixed-Mode Faults models, and we advocate that a similar approach can be adopted in order to prove the correctness of other classical distributed building blocks (e.g. agreement, clock synchronization, interactive consistency etc) under Mobile Byzantine Faults model.

==> problem.tex <==
%\begin{itemize}
%\item Agreement : The maximum difference between the values chosen by the correct nodes at the end of the iteration t should be strictly smaller than the maximum difference between the iteration t input values or be equal to the latter difference if it is zero.
%\item Validity : There is an iteration t such that for any iteration $t^\prime>t$ the "output" of correct nodes converges to the same value.   
%\end{itemize}

%Idea of the algorithm with asymmetric Byzantines :
%\begin{itemize}
%\item Garay : send to all, receive from all, remove the smallest f and biggest f and take the average on the rest (expected bound 4f+1)
%\item Sasaki the same as Garay except that I remove 2f on each side (expected bound 6f+1)
%\item Bonnet the same as Garay except that I remove 2f on each side (expected bound 4f+1 or 5f+1 ??? need to check why there is a difference with the formula !!!)
%\item Burman send to all, receive from all, remove the smallest f and biggest f and take the average on the rest (expected bound 3f+1)
%\end{itemize}

%Idea of the algorithm with symmetric Byzantines :
%\begin{itemize}
%\item Garay : send to all, receive from all, remove the smallest f and biggest f and take the average on the rest (expected bound 3f+1)
%\item Sasaki the same as Garay except that I remove 2f on each side (expected bound 4f+1)
%\item Bonnet the same as Garay except that I remove 2f on each side (expected bound 4f+1)
%\item Burman send to all, receive from all, remove the smallest f and biggest f and take the average on the rest (expected bound 2f+1)
%\end{itemize}

%A mix between Dolev, Garay and Bonnet properties.\\
As defined in \cite{LSP82}, each process starts with a value $v \in \mathbb{R}$. For a fixed $\epsilon$ (small as desired), an approximate agreement algorithm must satisfy the following properties:\\
\\
\noindent {\bf Agreement}: The voting algorithms executed by all non-faulty processes eventually return voted values that are within $\epsilon$ of each other.\\
\\
\noindent {\bf Validity}: The value returned by each non faulty process must be in the range of initial values of the non faulty processes.\\


